OptTyper: Probabilistic Type Inference by Optimising Logical and Natural Constraints

We present a new approach to the type inference problem for dynamic languages. Our goal is to combine \emph{logical} constraints, that is, deterministic information from a type system, with \emph{natural} constraints, that is, uncertain statistical information about types learnt from sources like identifier names. To this end, we introduce a framework for probabilistic type inference that combines logic and learning: logical constraints on the types are extracted from the program, and deep learning is applied to predict types from surface-level code properties that are statistically associated. The foremost insight of our method is to constrain the predictions from the learning procedure to respect the logical constraints, which we achieve by relaxing the logical inference problem of type prediction into a continuous optimisation problem. We build a tool called OptTyper to predict missing types for TypeScript files. OptTyper combines a continuous interpretation of logical constraints derived by classical static analysis of TypeScript code, with natural constraints obtained from a deep learning model, which learns naming conventions for types from a large codebase. By evaluating OptTyper, we show that the combination of logical and natural constraints yields a large improvement in performance over either kind of information individually and achieves a 4% improvement over the state-of-the-art.

==> figs/example/arrow1.tex <==
\scriptsize
\begin{tabular}[t]{l}
Inject Code with\\
Type Parameters
\end{tabular}

==> figs/example/arrow2.tex <==
\scriptsize
\begin{tabular}[t]{@{}c@{}}
Continuous Space
\end{tabular}

==> figs/example/arrow3.tex <==
\scriptsize
\begin{tabular}[t]{@{}c@{}}
Logical Constraints
\end{tabular}

==> figs/example/arrow4.tex <==
\scriptsize
\begin{tabular}[t]{@{}c@{}}
Natural Constraints
\end{tabular}

==> figs/example/arrow5.tex <==
\scriptsize
\begin{tabular}[t]{l}
Logical Constraints Relaxation
\end{tabular}

==> figs/example/caption2.tex <==
\scriptsize
\begin{tabular}[t]{l}
	(a) A minimal function with unknown type signature.
\end{tabular}

==> figs/example/caption3.tex <==
\scriptsize
\begin{tabular}[t]{l}
	(b) Probability matrix $P = [\bm{p}_1, \ldots, \bm{p}_V]^\mathsf{T}$, $T=V=3$.
\end{tabular}

==> figs/example/caption4.tex <==
\scriptsize
\begin{tabular}[t]{l}
	(c) Generated logical constraints for type parameters \\
	\ \ \ \ \ and their corresponding relaxation.
\end{tabular}

==> figs/example/caption5.tex <==
\scriptsize
\begin{tabular}[t]{l}
 (d) Prob. matrix \tiny $\mathcal{M}=[\bm{\mu}_1,\ldots, \bm{\mu}_V]^\mathsf{T}.$
\end{tabular}

==> figs/example/caption6.tex <==
\scriptsize
\begin{tabular}[t]{l}
	(e) Prob. matrix P after optimisation.
\end{tabular}

==> figs/example/caption7.tex <==
\scriptsize
\begin{tabular}[t]{l}
	(f) Combined probability matrix.
\end{tabular}

==> figs/example/caption8.tex <==
\scriptsize
\begin{tabular}[t]{l}
	(g) Resulting typed annotated code.
\end{tabular}

==> figs/example/code1.tex <==
\scriptsize\begin{tabular}[t]{>{\ttfamily}l}
\textcolor{myrose}{function} \textcolor{black}{addNum} (\textcolor{black}{start}, \textcolor{black}{end}) \{ \\
\ \ \ \ \textcolor{myrose}{var} \textcolor{black}{addN} = \textcolor{black}{start} + \textcolor{black}{end};\\
\ \ \ \ \textcolor{myrose}{return} \textcolor{black}{addN};\\
\}
\end{tabular}

==> figs/example/code2.tex <==
\scriptsize\begin{tabular}[t]{>{\ttfamily}l}
\textcolor{myrose}{function} \textcolor{RoyalBlue}{addNum}<\textcolor{mygreen}{START}, \textcolor{mygreen}{END}, \textcolor{mygreen}{ADDNUM}> ( \\
\ \ \textcolor{RoyalBlue}{start}: \textcolor{mygreen}{START}, \textcolor{RoyalBlue}{end}: \textcolor{mygreen}{END}): \textcolor{mygreen}{ADDNUM} \{ \\
\ \ \ \ \textcolor{myrose}{var} \textcolor{RoyalBlue}{addN} = \textcolor{RoyalBlue}{start} + \textcolor{RoyalBlue}{end};\\
\ \ \ \ \textcolor{myrose}{return} \textcolor{RoyalBlue}{addN};\\
\}
\end{tabular}

==> figs/example/code3.tex <==
\renewcommand{\arraystretch}{0.5}
\scriptsize
\begin{tabular}{@{}l@{\hskip 1mm} c@{\hskip 1mm} c@{\hskip 1mm} c@{}}
\toprule\\
Variable & \multicolumn{3}{c}{Type}\\ 
\cmidrule(l){2-4}
& $l_1$: \textbf{\textcolor{Maroon}{number}} \ & $l_2$: \textbf{\textcolor{Maroon}{string}} \ & $l_T$: \textbf{\textcolor{Maroon}{any}}\\ 
\midrule\\
$x_1$: \textbf{\textcolor{mygreen}{START}} & $p_{1,1}$ & $p_{1,2}$ & $p_{1,T}$\\
$x_2$: \textbf{\textcolor{mygreen}{END}} & $p_{2,1}$ & $p_{2,2}$ & $p_{2,T}$\\
$x_V$: \textbf{\textcolor{mygreen}{ADDNUM}} & $p_{V,1}$ & $p_{V,2}$ & $p_{V,T}$\\
\bottomrule
\end{tabular}


==> figs/example/code4.tex <==
\renewcommand{\arraystretch}{1.0}
\scriptsize
\begin{tabular}{@{}c@{}}
$E  = [(\textbf{\textcolor{mygreen}{START}} \mathrel{is} \textbf{\textcolor{Maroon}{number}}) \mathrel{and} (\textbf{\textcolor{mygreen}{END}} \mathrel{is} \textbf{\textcolor{Maroon}{number}})]$\\
$\mathrel{or}$\\
$[(\textbf{\textcolor{mygreen}{START}} \mathrel{is} \textbf{\textcolor{Maroon}{string}}) \mathrel{and} (\textbf{\textcolor{mygreen}{END}} \mathrel{is} \textbf{\textcolor{Maroon}{string}})]$
\end{tabular}


==> figs/example/code5.tex <==
\renewcommand{\arraystretch}{0.5}
\scriptsize
\begin{tabular}{@{}l c@{\hskip 1mm} c@{\hskip 1mm} c@{}}
\toprule
& \textbf{\textcolor{Maroon}{number}} & \textbf{\textcolor{Maroon}{string}} & \textbf{\textcolor{Maroon}{any}}\\ 
\midrule
\textbf{\textcolor{mygreen}{START}} & \textbf{0.84} & 0.11 & 0.05\\
\textbf{\textcolor{mygreen}{END}} & \textbf{0.60} & 0.08 & 0.32\\
\textbf{\textcolor{mygreen}{ADDNUM}} & \textbf{0.82} & 0.14 & 0.04\\
\bottomrule
\end{tabular}


==> figs/example/code6.tex <==
\renewcommand{\arraystretch}{0.5}
\scriptsize
\begin{tabular}{@{}l c@{\hskip 1mm} c@{\hskip 1mm} c@{}}
\toprule
& \textbf{\textcolor{Maroon}{number}} & \textbf{\textcolor{Maroon}{string}} & \textbf{\textcolor{Maroon}{any}}\\ 
\midrule
\textbf{\textcolor{mygreen}{START}} & 0.05 & \textbf{0.93} & 0.02\\
\textbf{\textcolor{mygreen}{END}} & 0.06 & \textbf{0.93} & 0.01\\
\textbf{\textcolor{mygreen}{ADDNUM}} & 0.01 & 0.01 & \textbf{0.98}\\
\bottomrule
\end{tabular}


==> figs/example/code7.tex <==
\renewcommand{\arraystretch}{0.5}
\scriptsize
\begin{tabular}{@{}l c@{\hskip 1mm} c@{\hskip 1mm} c@{}}
\toprule
& \textbf{\textcolor{Maroon}{number}} & \textbf{\textcolor{Maroon}{string}} & \textbf{\textcolor{Maroon}{any}}\\ 
\midrule
\textbf{\textcolor{mygreen}{START}} & \textbf{0.90} & 0.07 & 0.03\\
\textbf{\textcolor{mygreen}{END}} & \textbf{0.86} & 0.05 & 0.09\\
\textbf{\textcolor{mygreen}{ADDNUM}} & \textbf{0.83} & 0.14 & 0.03\\
\bottomrule
\end{tabular}


==> figs/example/code8.tex <==
\scriptsize\begin{tabular}[t]{>{\ttfamily}l}
\textcolor{myrose}{function} \textcolor{RoyalBlue}{addNum}(\textcolor{RoyalBlue}{start}: \textcolor{Maroon}{number},\\
\ \ \textcolor{RoyalBlue}{end}: \textcolor{Maroon}{number}): \textcolor{Maroon}{number}
\end{tabular}

==> figs/example/eqC.tex <==
\scriptsize
\begin{tabular}{@{}l@{}}
$\underset{P}{\mathrm{min}} \sum_v || \bm{p}_v - \bm{\mu}_v ||_2^2 -\lambda \qqpi{P}{E}$
\end{tabular}

==> figs/example/eqE.tex <==
\scriptsize
\begin{tabular}{@{}c@{}}
$\qqpi{P}{E} = \left( p_{1,1} \mathrel{*} p_{2,1} \right) \mathrel{+} \left( p_{1,2} \mathrel{*} p_{2,2} \right) \mathrel{-}$\\
\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ $[ \left(p_{1,1} \mathrel{*} p_{2,1}\right) \mathrel{*} \left(p_{1,2} \mathrel{*} p_{2,2}\right)]$
\end{tabular}

==> figs/example/text1.tex <==
\scriptsize
\begin{tabular}{@{}c@{}}
	       Untyped Code
\end{tabular}

==> figs/example/text2.tex <==
\scriptsize
\begin{tabular}{@{}c@{}}
	  Typed Code
\end{tabular}
